Deep Reinforcement Learning solution for pickup and delivery routing problems with time window and capacity constraints

The task of constructing vehicles optimal routes for pickup and delivery of goods is one of most promising tasks in the context of global urban population growth. Although this kind of problems with small size can be solved by various classical approaches, a fast (or realtime) route optimizer under the constraints of the real world (such as capacity and time windows constraints) for medium-large size problems still remains a highly challenging task. In this work we, for the first time, successfully applied a deep Reinforcing Learning approach (modified JAMPR model) to solve Pickup and Delivery problem with Capacity and Time Window constraints (CPDPTW). We obtained a robust model that gives a fast optimal solution for problems of small and medium size, and gives fast suboptimal solution for problems of larger (> 200) size.

==> Makefile <==
MAIN := samplepaper.tex
JOB := CPDPTW_Deep_RL_English
BUILD_DIR := tmp/pdfs/build
OUTPUT_DIR := output/pdf
PDF := $(OUTPUT_DIR)/$(JOB).pdf

.PHONY: all pdf clean

all: pdf

pdf:
	mkdir -p $(BUILD_DIR) $(OUTPUT_DIR)
	latexmk -pdf -interaction=nonstopmode -halt-on-error -file-line-error \
		-outdir=$(BUILD_DIR) -jobname=$(JOB) $(MAIN)
	cp $(BUILD_DIR)/$(JOB).pdf $(PDF)

clean:
	latexmk -C -outdir=$(BUILD_DIR) -jobname=$(JOB) $(MAIN)
	rm -rf $(BUILD_DIR)
	rm -rf tmp/pdfs/rendered
	rm -f *-eps-converted-to.pdf

